Sibylvariant Transformations for Robust Text Classification

The vast majority of text transformation techniques in NLP are inherently limited in their ability to expand input space coverage due to an implicit constraint to preserve the original class label. In this work, we propose the notion of sibylvariance (SIB) to describe the broader set of transforms that relax the label-preserving constraint, knowably vary the expected class, and lead to significantly more diverse input distributions. We offer a unified framework to organize all data transformations, including two types of SIB: (1) Transmutations convert one discrete kind into another, (2) Mixture Mutations blend two or more classes together. To explore the role of sibylvariance within NLP, we implemented 41 text transformations, including several novel techniques like Concept2Sentence and SentMix. Sibylvariance also enables a unique form of adaptive training that generates new input mixtures for the most confused class pairs, challenging the learner to differentiate with greater nuance. Our experiments on six benchmark datasets strongly support the efficacy of sibylvariance for generalization performance, defect detection, and adversarial robustness.

==> _experiments.tex <==
\section{Experiments}
\label{experiments}

% OLD INTRO
% In order to determine the extent to which sibylvariance can create effective tests which detect model defects and generate new training data that improves model performance, we investigate our three research questions. We empirically validate the proposed framework by \emph{a)} exploring natural language processing tasks and \emph{b)} focusing on the performance of classification models trained on labeled datasets augmented with our functions and others used in practice.

% We experimentally study our unified framework for data transformations

%\subsection{Datasets.} 
 % \mknote{FHC, How is 144 calculated?} \fhnote{144 = 6 datasets x 3 different numbers of classes x 8 different TPs. NOTE: We study 11 TPs in total, 6 x 3 x 11 = 198 different experimental configurations. However, 3 of them are adaptive pipelines and we don't create / store that data - it is generated at run-time and then discarded.}


\subsection{Transformation Pipelines.} 

To evaluate the impact of each transformation kind such as INV, SIB, or INVSIB, we construct a {\em transformation pipeline}  (TP)~\cite{randaugment, uda}, where we uniformly sample $n$ transformations of the selected kind to construct $\{X_i,y_i\}$ pairs. TP measures the impact of INV,  SIB, or INVSIB in aggregate. We also construct TPs that applies a single transformation  in isolation, $T_{\texttt{SINGLE}}$, to highlight the effect of {\tt C2S}, {\tt TextMix}, {\tt SentMix}, {\tt WordMix} and adaptive training of the three mixture mutations: {\tt $\alpha$TextMix}, {\tt $\alpha$SentMix}, and {\tt $\alpha$WordMix}. In total, we evaluate 11 $TP$s per dataset, shown in Table \ref{tab:trans_pipelines}. 

We use six benchmark NLP datasets for two kinds of tasks: topic classification and sentiment analysis. Table \ref{tab:datasets} summarizes results, when varying the number of examples per class --- 10, 200, 2500. Each class-balanced dataset was then transformed via a given TP 30 times, meaning that we repeat the process of applying a randomly chosen transformation of the given kind 30 times. By retaining the original data and adding new transformed data, we investigate the effectiveness of data {\em augmentation} as opposed to data {\em replacement}.  In total, we generated 144 versions (144=6*3*8, where 6 benchmarks, 3 example sizes, and 8 different persisted data-sets). 

To compare the potential of INV~vs~SIB, Table~\ref{tab:datasets} reports a top performing TP of each kind using an asterisk (*).  For example, INV* represents the best result from $T_{\text{INV}}$ or $T_{\texttt{C2S}}$), while SIB* represents the best result from $T_{\text{SIB}}$ or other mixture mutations. Appendix~\cite{} has the full results. 

\begin{table}[h]
    \centering
    \begin{tabular}{l p{5cm}}
        \toprule
        \textbf{Shorthand} & \textbf{Description}             \\
        \midrule
        $T_{\text{ORIG}}$      & 0 transformations as baseline     \\
        $T_{\text{INV}}$       & sample 2 INVs             \\
        $T_{\text{SIB}}$       & sample 2 SIBs             \\
        $T_{\text{INVSIB}}$    & sample 1 INV and 1 SIB    \\
        $T_{\text{SINGLE}}$  & apply 1 transformation in isolation from C2S, TextMix, SentMix, WordMix, $\alpha$TextMix, $\alpha$SentMix, or $\alpha$WordMix \\
        \midrule
    \end{tabular}
    \caption{TP with the $\alpha$ prefix uses targeted, adaptive training by monitoring confusion matrix in each mini batch in Section \ref{ada}.}
    \label{tab:trans_pipelines}
    \vspace{-1.25em}
\end{table}

% \mknote{This table is gigantic and overwhelming in my opinion. It's not easy to see the high level mgs here.}  


\begin{table*}[h]
    \centering
    \begin{tabular}{l l l l c c}
        \toprule
        \textbf{Dataset} & \textbf{Source}         & \textbf{Task Type} & \textbf{Subject}      & \textbf{Classes}  & \textbf{Test} \\
        \midrule
        AG News          & \cite{CCN_datasets}     & Topic              & News Articles         & 4                 &  1,900    \\
        DBpedia          & \cite{CCN_datasets}     & Topic              & Wikipedia Articles    & 14                &  5,000    \\
        Yahoo! Answers   & \cite{CCN_datasets}     & Topic              & QA Posts                   & 10                &  6,000    \\
        Yelp Polarity    & \cite{CCN_datasets}     & Sentiment          & Business Reviews      & 2                 &  10,000   \\
        Amazon Polarity  & \cite{CCN_datasets}     & Sentiment          & Product Reviews       & 2                 &  200,000  \\
        IMDB             & \cite{IMDB}             & Sentiment          & Movies Reviews        & 2                 &  12,500   \\
        \midrule
    \end{tabular}
    \caption{Dataset details. Test represents the number of examples per class in the test set. } 
    \label{tab:datasets}
\end{table*}

\subsection{Model Setting}

We used a \texttt{bert-base-uncased} model / tokenizer \cite{BERT} as implemented in Huggingface \cite{huggingface} with average pooling over the output of the encoder, followed by a dropout layer \cite{dropout} with probability $0.1$, and a single linear layer with hidden size 768 and GELU \cite{gelu} activation. Maximum sentence length was set to 250 to maintain reasonable training times. We use a batch size of $16$, an Adam optimizer \cite{adam} with a linear warmup over one epoch, a $0.1$ weight decay, and compute validation every $2,000$ steps. All models were trained for $30$ epochs on an array of eight Nvidia RTX A6000 GPUs, with early stopping if validation accuracy could not be improved after $10$ evaluation cycles. In total, the experiments required 198 different models to be constructed. 

For all $TP$s which produce a soft-label, we use a multi-class cross-entropy loss and  computed performance via a weighted top-k accuracy,
\begin{equation}
    \sum_j^k \lambda_j \cdot \mathbbm{1}(y_j = \hat{y}_j),
\end{equation}
where $\lambda_j$ is the degree (weight) of class membership, $\mathbbm{1}(\cdot)$ is the indicator function, and $y_j$ and $\hat{y}_j$ are the indices of the $j$-th largest predicted score for the ground truth label and predicted label, respectively. For example, if a model predicted $[0.5, 0.1, 0.4]$ for the label $[0.7, 0.3, 0.0]$ and $k=2$, the weighted top-k accuracy is $0.7$ because the first index correctly overlaps, but the others do not.

\subsection{Results}

\subsubsection{RQ1. Generalization Performance}
\label{RQ1}

For this RQ, we explore how model accuracy on the original test set is influenced by training data augmented with our INV and SIB $TP$s. Table \ref{tab:train_acc} shows the performance on the six classification datasets and three levels of data availability. The baselines are ORIG and TMix \cite{mixtext}, a recently proposed latent-space mixture mutation. 

We observed the most significant performance gains in the low-resource setting of only 10 examples per class where accuracy was improved by 4.7\% on average across all datasets and by a maximum of up to 15\% for IMDB. As the number of labeled training data increases, a dominant trend emerged where a sibylvariant $TP$ always generalized better to the unseen test data. In fact, the only type of transformation to always outperform both baselines was sibylvariant one.  

One of the key ingredients that aided SIB transformations in attaining this strong performance was use of our adaptive training routine. On average, crafting new examples that targeted the model's primary confusions during training added approximately 1\% to test accuracy relative to the same transformations mixing classes uniformly at random. This result demonstrates another unique benefit of our sibylvariant framework that is not transferable to their invariant counterparts. 

% By the end of training, the targeted models will have seen more examples of the kinds of inputs they find most challenging to differentiate. This generally allows them to refine their decision boundary in a more efficient manner than the simpler random sampling strategy used by the untargeted transforms. 

% \mknote{1st paragraph on detailed results for 200 examples. the key msg is that SIB does better than INV or ORG. So Figure 1 (Detail Result) for the results of 200 tells the detailed story of how each transformation does for ORG INV, SIV and INVSIV. I am okay with 4 bars or 8 bars }
% \fhnote{Since our largest increases are for the 10-per-class case, I think its important to show those. However, for that number of examples, INV* is better 2 out of 6 times. To counteract that, we'd have to show all the results to reinforce the strength of SIB*, which is best 16 out of 18 times. Then with all the data upfront, we wouldn't need to show the scaling table. }

% \mknote{2nd paragraph, scaling: Table 2 (Scaling) is an aggregate table to show that  how ORG, INV, SIV and INVSIV does, as we increase \# of examples.} 

% \mknote{3rd paragraph, which SIB transformation does best and how much. Table 3 (Top one and delta) is to show all six data sets, what are the top performing transformation and how much delta it has from INV or ORG. Its message is to show that “some kind of MIX” is a top performing one  in 5 out of 6 data sets and it has decent margin / delta from ORG and INV.}

% \begin{figure}[htbp]
%     \centering
%     \begin{subfigure}[b]{0.23\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{imgs/v2/train_acc_ag_news.png}
%         \caption{AG News}
%         \label{fig:test_acc_ag_news}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.23\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{imgs/v2/train_acc_dbpedia_14.png}
%         \caption{DBpedia}
%         \label{fig:test_acc_dbpedia_14}
%     \end{subfigure}
%     \\
%     \begin{subfigure}[b]{0.23\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{imgs/v2/train_acc_yahoo_answers_topics.png}
%         \caption{Yahoo! Answers}
%         \label{fig:test_acc_yahoo_answers_topics}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.23\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{imgs/v2/train_acc_imdb.png}
%         \caption{IMDB}
%         \label{fig:test_acc_imdb}
%     \end{subfigure}
%     \\
%     \begin{subfigure}[b]{0.23\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{imgs/v2/train_acc_amazon_polarity.png}
%         \caption{Amazon Polarity}
%         \label{fig:test_acc_yahoo_amazon_polarity}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.23\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{imgs/v2/train_acc_yelp_polarity.png}
%         \caption{Yelp Polarity}
%         \label{fig:test_acc_yelp_polarity}
%     \end{subfigure}
%     \caption{Performance (test set accuracy) comparisons when trained on 10 examples of each class. The annotated figures shows the percent change in accuracy relative to $T_{\texttt{ORIG}}$.}
%     \label{fig:test_acc}
% \end{figure}

\begin{table*}[htbp]
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
    \cline{1-5} \cline{7-11}
    \textbf{dataset}                                                                    & \textbf{transform} & \textbf{10}    & \textbf{200}   & \textbf{2500}  & \multirow{16}{*}{\textbf{}} & \textbf{dataset}                                                                    & \textbf{transform} & \textbf{10}    & \textbf{200}   & \textbf{2500}  \\ \cline{1-5} \cline{7-11} 
    \multirow{5}{*}{\textbf{AG News}}                                                   & ORIG               & 75.08          & 88.70          & 91.65          &                             & \multirow{5}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Amazon\\ Polarity\end{tabular}}} & ORIG               & 67.30          & 89.22          & 92.08          \\ \cline{2-5} \cline{8-11} 
                                                                                        & INV*               & \textbf{84.28} & 89.46          & 91.95          &                             &                                                                                     & INV*               & 73.69          & 89.53          & 92.21          \\ \cline{2-5} \cline{8-11} 
                                                                                        & SIB*               & 83.52          & \textbf{89.80} & \textbf{92.42} &                             &                                                                                     & SIB*               & \textbf{74.90} & \textbf{90.03} & \textbf{92.26} \\ \cline{2-5} \cline{8-11} 
                                                                                        & INVSIB             & 84.09          & 89.00          & 91.36          &                             &                                                                                     & INVSIB             & 73.50          & 89.06          & 91.26          \\ \cline{2-5} \cline{8-11} 
                                                                                        & TMix               & 81.38          & 88.62          & 89.43          &                             &                                                                                     & TMix               & 62.14          & 87.98          & 91.00          \\ \cline{1-5} \cline{7-11} 
    \multirow{5}{*}{\textbf{DBpedia}}                                                   & ORIG               & 95.71          & 98.87          & 98.96          &                             & \multirow{5}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Yelp\\ Polarity\end{tabular}}}   & ORIG               & 74.62          & 91.66          & 93.70          \\ \cline{2-5} \cline{8-11} 
                                                                                        & INV*               & 97.29          & 98.81          & 99.00          &                             &                                                                                     & INV*               & \textbf{83.91} & 92.00          & 94.29          \\ \cline{2-5} \cline{8-11} 
                                                                                        & SIB*               & \textbf{97.96} & \textbf{98.90} & \textbf{99.06} &                             &                                                                                     & SIB*               & 80.46          & \textbf{92.60} & \textbf{94.69} \\ \cline{2-5} \cline{8-11} 
                                                                                        & INVSIB             & 95.64          & 98.74          & 98.92          &                             &                                                                                     & INVSIB             & 78.90          & 91.85          & 93.03          \\ \cline{2-5} \cline{8-11} 
                                                                                        & TMix               & 95.76          & 98.53          & 98.55          &                             &                                                                                     & TMix               & 61.81          & 91.19          & 92.80          \\ \cline{1-5} \cline{7-11} 
    \multirow{5}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Yahoo! \\ Answers\end{tabular}}} & ORIG               & 56.24          & 69.77          & 73.18          &                             & \multirow{5}{*}{\textbf{IMDB}}                                                      & ORIG               & 64.70          & 86.96          & 90.02          \\ \cline{2-5} \cline{8-11} 
                                                                                        & INV*               & 61.39          & 69.21          & 72.53          &                             &                                                                                     & INV*               & 76.20          & 86.94          & 89.69          \\ \cline{2-5} \cline{8-11} 
                                                                                        & SIB*               & \textbf{62.47} & \textbf{70.10} & \textbf{73.37} &                             &                                                                                     & SIB*               & \textbf{79.74} & \textbf{87.65} & \textbf{90.90} \\ \cline{2-5} \cline{8-11} 
                                                                                        & INVSIB             & 62.01          & 67.75          & 73.16          &                             &                                                                                     & INVSIB             & 75.04          & 87.04          & 88.24          \\ \cline{2-5} \cline{8-11} 
                                                                                        & TMix               & 53.68          & 69.03          & 69.50          &                             &                                                                                     & TMix               & 62.45          & 86.94          & 88.29          \\ \cline{1-5} \cline{7-11} 
    \end{tabular}%
    }
    \caption{Performance (test set accuracy (\%)) for variant types plus ORIG and TMix baselines for comparison. The results are averaged across three runs. Models are trained with either 10, 200, or 2500 examples per class. An asterisk (*) indicates the best performance observed across underlying $TP$s of that variant type.}
    \label{tab:train_acc}
\end{table*}


\subsubsection{RQ2. Defect Detection}
\label{RQ2}

% \mknote{now that we showed 3 sub figures for accuracy improvement, for this section, I think we can be brief. See the figure on your slack msg at 7:32 pm and my reply to it on 8:35pm on Sat.}
% \mknote{the key msg is that data aug with SIB can reveal defects (misclassifications) in models  detect better. I think we can pick ORG, SIB*, INV*, INVSIB and then in the text, you can name which specific transformation can detect defects best}
% \fhote{Since we presently have a table for RQ1, I'd like to keep the current plots to give the reader a break from tables. We can also keep the 8 TPs as is since it shouldn't be too overwhelming like the 12 TPs would be. }

For this RQ, we explore how generating new tests via INV and SIB transformations can expose differing amounts of defective model behavior. A single test is simply an $\{X_i,y_i\}$ pair and a test suite is a set of such tests. Defective behavior in this setting is misclassification and is measured via test suite accuracy. For each dataset, $D$, we selected a high-performing BERT model trained only on the original dataset without any augmentation. Then for each of eight $TP$s\footnote{Excluding 3 adaptive $TP$s relevant to training time only.}, we created 100 test suites each containing 100 randomly sampled tests for each dataset, yielding a total of 480,000 tests. We then report the average test suite accuracy per combination of $D$ and $TP$.

At a fundamental level, the value of any test is a function of its proximity to the program's expected input distribution. Tests which lie outside this domain are not likely to be considered either fair nor actionable. Since the space of natural language is intractably large, it is challenging to determine exactly where the boundaries exist for a given task's intended input space. We propose the following heuristic: if training on a set of $\{X_i,y_i\}$ pairs can improve model generalization performance on known, in-domain data, then the set can be considered a valid and useful test suite. Consequently, the positive results of the generalization study in \textbf{RQ1} supports the use of SIB transformations as reasonable for testing. After all, if sibylvariant transformations pushed the new data out of distribution, it is difficult to see how they would so consistently improve model accuracy on in-domain examples. 

\begin{figure}[htbp]
    \centering
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{imgs/v2/test_acc_ag_news.png}
        \caption{AG News}
        \label{fig:test_acc_ag_news}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{imgs/v2/test_acc_dbpedia_14.png}
        \caption{DBpedia}
        \label{fig:test_acc_dbpedia_14}
    \end{subfigure}
    \\
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{imgs/v2/test_acc_yahoo_answers_topics.png}
        \caption{Yahoo! Answers}
        \label{fig:test_acc_yahoo_answers_topics}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{imgs/v2/test_acc_imdb.png}
        \caption{IMDB}
        \label{fig:test_acc_imdb}
    \end{subfigure}
    \\
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{imgs/v2/test_acc_amazon_polarity.png}
        \caption{Amazon Polarity}
        \label{fig:test_acc_yahoo_amazon_polarity}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{imgs/v2/test_acc_yelp_polarity.png}
        \caption{Yelp Polarity}
        \label{fig:test_acc_yelp_polarity}
    \end{subfigure}
    \caption{Average test suite accuracy for all models by $TP$ and dataset. The annotated figures shows the percent change in accuracy relative to $T_{\texttt{ORIG}}$.}
    \label{fig:test_acc}
\end{figure}

Figure \ref{fig:test_acc} shows how classification accuracy is influenced by our INV and SIB transformations. With the exception of Yahoo! Answers, the models scored nearly perfect accuracy on the $T_{\text{ORIG}}$ test suites; however when we test the models on our transformed suites, it revealed that they still struggled to generalize to other valid portions of their expected input spaces. Additionally, the greatest decreases in accuracy were observed for SIB test suites, indicating the value of our {\em sibylvariant} approach to testing ML models in the absence of human judgements.

We theorize that the increased effectiveness of sibylvariance comes from the wider range of testing objectives they permit. For example, $T_{\text{TextMix}}$ constructs a deliberately blended input to assess whether the model can recognize which classes are represented and to what degree. $T_{\text{SentMix}}$ does the same, but emphasizes long-range comprehension by broadly distributing related topic sentences. Datasets with lengthy inputs are particularly vulnerable to transformations of this kind. Lastly, $T_{\text{WordMix}}$ forces the model to forgo reliance on text structure and evaluates keyword comprehension amidst noisy contexts. In contrast, most invariant transforms involve minor changes --- e.g. expand contractions --- and test elements of language already well modeled from extensive pre-training in modern models. Our invariant C2S transform is an exception that more drastically alters the form of the input and thus reveals more defects than the standard $T_{\text{INV}}$ pipeline across all datasets. 

\subsubsection{RQ3. Adversarial Robustness}
\label{RQ3}

For this RQ, we explore whether models trained on INV or SIB augmented datasets are more or less resilient to adversarial attacks than models trained on an original dataset. An adversarial text input is typically obtained via semantic preserving (i.e. \emph{invariant}) perturbations to legitimate examples in order to deteriorate the performance of the model. The changes are typically generated by ascending the gradient of the loss surface with respect to the original example and improving robustness to such attacks is a necessary precondition for real-world deployment of NLP technologies.

We selected three attack algorithms based on their popularity and published effectiveness: (1) TextFooler \cite{textfooler}, (2) DeepWordBug \cite{deepwordbug}, and (3) TextBugger \cite{textbugger}, all as implemented in TextAttack \cite{textattack}. We focused this study on models trained with 10 examples per class because the largest changes in generalization performance are more likely to exhibit the clearest trends for adversarial robustness. For each of 11 models and 3 attacks, we randomly sampled 100 inputs from the original test set to perturb into a total of 3,300 adversarial examples. The results of this study are summarized in Table \ref{tab:adv_robustness} and a full breakdown by $TP$ is available in the appendix. 

Of all the cases where adversarial robustness was improved over the $T_{\texttt{ORIG}}$ baseline, 92\% of them involved sibylvariant transformations. On average, the SIB*-trained models improved robustness by 4\%, while the INV*-trained models sustained a 1\% decrease. Topic classification datasets were made more consistently robust via training on augmented data, and $T_{\texttt{Ada-SentMix}}$ in particular always discovered the most resilient models. For sentiment analysis, most models were more vulnerable to attacks. This surprising result raised a new question about the relationship between generalization performance and adversarial robustness. The underlying sentiment models trained with augmented datasets improved generalization over $T_{\texttt{ORIG}}$ by an average of 5\%, which should have jointly improved resistance to attacks given the better domain space representation. Counterintuitively, we observed a modest Pearson correlation of -0.28 between accuracy on the test set and robustness across all three attacks. This finding motivates future work to both characterize and disentangle the two objectives within the domain of natural language. 

% \mknote{I suggest we also pick which transformation is the most robust to each adversarial attack algorithmm and present the delta: 
% Then for all six data sets, we can only pick the top performing ones  and just name the transformation (such as TexMix) that is responsible for the top one, and how much difference it has from ORG or INV. So the message that I want to send is that MIX transformation tends to be a top performing one, but this is not always consistent across different data set and that when accuracy is improved, adversarial robustness is not improved together.}

% \mknote{describe your key take away msg that more future work is necessary to investigate why adversarial robustness is not improved, when accuracy is improved. put a positive spin}

\begin{table*}[htbp]
    \centering
    % \resizebox{\textwidth}{!}{%
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
    \cline{1-5} \cline{7-11}
    \textbf{Dataset}                                                                    & \textbf{TP} & \textbf{TF} & \textbf{DWB} & \textbf{TB} & \multirow{13}{*}{\textbf{}} & \textbf{Dataset}                                                                    & \textbf{TP} & \textbf{TF} & \textbf{DWB} & \textbf{TB} \\ \cline{1-5} \cline{7-11} 
    \multirow{4}{*}{\textbf{AG News}}                                                   & ORIG        & 0.69                & 0.56                 & 0.54                &                             & \multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Amazon\\ Polarity\end{tabular}}} & ORIG        & \textbf{0.48}       & 0.40                 & 0.42                \\ \cline{2-5} \cline{8-11} 
                                                                                        & INV*        & 0.66                & 0.56                 & 0.48                &                             &                                                                                     & INV*        & 0.49                & 0.42                 & \textbf{0.36}       \\ \cline{2-5} \cline{8-11} 
                                                                                        & SIB*        & \textbf{0.60}       & \textbf{0.43}        & \textbf{0.45}       &                             &                                                                                     & SIB*        & 0.55                & \textbf{0.39}        & 0.46                \\ \cline{2-5} \cline{8-11} 
                                                                                        & INVSIB      & 0.78                & 0.62                 & 0.57                &                             &                                                                                     & INVSIB      & 0.65                & 0.58                 & 0.60                \\ \cline{1-5} \cline{7-11} 
    \multirow{4}{*}{\textbf{DBpedia}}                                                   & ORIG        & 0.92                & 0.55                 & 0.64                &                             & \multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Yelp\\ Polarity\end{tabular}}}   & ORIG        & \textbf{0.48}       & \textbf{0.20}        & \textbf{0.28}       \\ \cline{2-5} \cline{8-11} 
                                                                                        & INV*        & \textbf{0.76}       & 0.47                 & 0.48                &                             &                                                                                     & INV*         & 0.64                & 0.41                 & 0.52                \\ \cline{2-5} \cline{8-11} 
                                                                                        & SIB*        & 0.77                & \textbf{0.40}        & \textbf{0.41}       &                             &                                                                                     & SIB*         & 0.61                & 0.39                 & 0.53                \\ \cline{2-5} \cline{8-11} 
                                                                                        & INVSIB      & 0.83                & 0.56                 & 0.52                &                             &                                                                                     & INVSIB      & 0.75                & 0.51                 & 0.61                \\ \cline{1-5} \cline{7-11} 
    \multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Yahoo! \\ Answers\end{tabular}}} & ORIG        & 0.54                & 0.46                 & 0.52                &                             & \multirow{4}{*}{\textbf{IMDB}}                                                      & ORIG        & 0.86                & \textbf{0.25}        & 0.71                \\ \cline{2-5} \cline{8-11} 
                                                                                        & INV*        & 0.57                & 0.49                 & 0.49                &                             &                                                                                     & INV*        & 0.70                & 0.50                 & 0.68                \\ \cline{2-5} \cline{8-11} 
                                                                                        & SIB*        & \textbf{0.48}       & \textbf{0.41}        & 0.49                &                             &                                                                                     & SIB*        & \textbf{0.56}       & 0.32                 & \textbf{0.55}       \\ \cline{2-5} \cline{8-11} 
                                                                                        & INVSIB      & 0.54                & 0.44                 & \textbf{0.46}       &                             &                                                                                     & INVSIB      & 0.89                & 0.79                 & 0.88                \\ \cline{1-5} \cline{7-11} 
    \end{tabular}%
    % }
    \caption{Attack success by dataset and variant type for three adversarial algorithms: TextFooler (TF), DeepWordBug (DWB), and TextBugger (TB). Lower attack success indicates higher adversarial robustness.}
    \label{tab:adv_robustness}
\end{table*}



==> _intro.tex <==
\section{Introduction}
\label{introduction}

Automatically generating new data is a critical component within modern machine learning pipelines. During training, data augmentation can expose models to a larger portion of their potential input space, consistently leading to better generalization and performance \cite{trans_inv, alexnet, effectiveness_da}. After training, creating effective test instances from existing data can expose specific model failure modes and provide actionable corrective feedback \cite{ml_test_survey, checklist}. 

While many existing techniques can artificially expand labeled training sets or test suites, nearly all of them are class-preserving. In other words, these transformations are invariant (INV) with respect to existing data, which could potentially amplify confounding factors in existing data and create data with skewed distribution of class labels. %\mknote{ not sure what this means---in an out-of-distribution null class which might impede the learning objective. However, it also necessitates the use of a smaller set of conservative transformations that inherently limit the degree of diversifying perturbations that can be injected into existing data.}  

In this work, we propose and investigate the potential of {\em sibylvariant (SIB) transformations} that {\em knowably} vary the expected class. This term is derived from the Greek word for oracles, \emph{sibyls}, as this problem has a parallel analogy the test oracle construction problem in software testing \cite{oracle_prob}. In a nutshell, SIB either fully transmutes a datum from one class $c_i$ to another $c_j$, or mixes data from multiple classes together to derive a new soft label that reflects the mixed membership. In this way, SIB  can increase the degree of perturbation and diversify underlying class label distribution. Moreover, SIB could enable a new type of adaptive training by synthesizing data with frequently confused class pairs and by challenging the model to differentiate with greater refinement. 

\mknote{this paragraph is currently repetitive. It should be re-written. please add one or two concrete examples of sybiltransformations}

To investigate the potential of SIB in NLP, we define a text data augmentation framework, called {\tool}. It currently provides 40 different kinds of transformations, each of which can serve the role of either INV or SIB for two different types of tasks: sentiment analysis and topic classification. SIB could be categorized into two categories. First, {\em transmutations} convert one discrete class label to another label. Second, {\em mixture mutations} blend two or more classes. For example, {\sf TextMix} is a transformation under the {mixture mutations} category that merges two input texts and interpolates a software label according to the proportion of tokens belonging to the constituent classes. As another example, {\sf SentMix} shuffles sentences to encourage long-range comprehension, as prediction-critical information may exist in several parts of the text. Compared to prior work~\cite{mixtext} \mknote{add citation here} that operates on the hidden space, all transformations in {\tool} operate in the input space to provide greater transparency and examinability. This poses more challenges because adding, replacing, and deleting words or sentences thus must adhere to the rules of grammar, style, etc. 

To comprehensive evaluate how SIB could complement INV transformations in data augmentation, we conduct a compherensive evaluation of these 40 different transformations. We use six different benchmarks (AG News, DBpedia, Yahoo! Answers, Yelp Polarity, and Amazon Polarity, and IMBD) on two different types of classification tasks (sentiment analysis and topic classification). For each benchmark, we then instantiate the total 12 pipelines by selecting which subset of data to be transformed and by systematically sampling different transformations to compare the potential of data augmentation: INV only, SIB only, INV and SIB together, and MIX-SIB only. {\tool} currently supports individual transformations in isolation and combines different transformations on the fly via uniform sampling~\cite{randaugment, uda}.  
\mknote{add a sentence on the total configuration. In total, our extensive experimentation generate X configurations of transformation pipelines, constructing X MB data}.  

We investigate the following three research questions.  \mknote{add some detailed summary of how extensive our experimental set up is. data sets, how many different data suites, (similar to our FSE paper that summarizes the total size of experimental condition) etc}. 

% % MK phrasing
% \begin{itemize}
%     \item\textbf{RQ1. Training Accuracy.} How much additional model accuracy improvement do sybylvariant transformations provide than using invariant transformations alone during training?    
%     \item\textbf{RQ2. Defect Detection.} How effective are the models re-trained with sybylvariant augmentation at detecting misclassifications during testing?
%     \item\textbf{RQ3. Adversarial Robustness.} How robust are the models re-trained with sybilvariant augmentation when attacking them using existing adversarial attack algorithms for text? 

%     %    \mknote{I do not understand your original question of 'what kinds or transformations are better at detecting defective behaviors?'I read the description in Sect 4.1 and still don't understand what you mean by defective behavior. Is it just Testing Accuracy?} \fhnote{Defective behaviors are defined as model errors (misclassifications), i.e. testing accuracy. The tested models are those trained on the ORIG dataset (no transforms), to see how well they handle the variation injected by Sibyl.} 
% \end{itemize} 

%FHC phrasing 
\mknote{FHC, we seem to dilute msgs by rephrasing SIB to INV or SIB? Even though the results are not all about SIB, we should pose questions that way? This should be about hypothesis. Not sure whether it helps with distilling key msg.}
\begin{itemize}
    \item\textbf{RQ1. Generalization Performance.} How does training on data {data augmented with SIB} improve model accuracy compared to INV on the original test set? 
    \item\textbf{RQ2. Defect Detection.} For models trained on the original dataset, how effective are tests generated by SIB for inducing misclassifications?  
    \item\textbf{RQ3. Adversarial Robustness.} Are models trained on SIB-augmented data more resistant to existing adversarial attack algorithms? 
\end{itemize} 

\mknote{add some crisp result summaries and take away msgs here.}
\mknote{example:In terms of how to summarize results, even if they are not all consistent and conclusive, I think we should try to say a little more specific way, such as X\% of experimental configurations, SIB outperform INV by Y\% in improving model accuracy, implying that SIB can effectively complement INV in augmenting training data. More specifically X, Y, and Z transformations are most effective…}

%Experimental results that can be seen in Section \ref{experiments} show that SIB transformations generally perform as well and often significantly better than INV methods at creating tests that expose model misbehavior and for improving accuracy via training. We then offer some points for discussion and potential threats to validity (Section \ref{discussion}) before positioning sibylvariance in the context of related work (Section \ref{related_work}). The source code for the \texttt{Sibyl} tool and our experiments is available at:

The rest of this paper is organized as follows. Section~\ref{sibylvariance} introduces the language necessary to taxonomize different types of data transformations. Section~\ref{transformations} overviews a set of text transformations that can serve the role of SIB and INV for different tasks using concrete examples. It also highlights novel text transformations we designed based on recent advances on natural language generation \mknote{such as XXX, name tool and add citation~\cite{}}. Section~\ref{experiments} discusses experimental results, including benchmarks, transformation pipelines, target models. Section~\ref{discussion} includes some rationale behind how and why SIB could complement INV.    
\mknote{Based on what we said on the phone, our results on accuracy improvement and robustness reduction is somewhat unintuitive yet interesting. I suggest that we write and summarize the results as is.} \fhnote{Agreed}  \begin{center}
    \url{https://zenodo.org/record/4835770} \fhnote{Replace this!}
    % \url{https://doi.org/10.5281/zenodo.4835770} % doesn't work for some reason...
    % \url{https://github.com/fabriceyhc/Sibyl}
\end{center}

% Experimental results suggest that SIB transformations perform significantly better than the INV methods that presently dominate industry practice and academic research.
